Polygon: Symbolic Reasoning for SQL using Conflict-Driven Under-Approximation Search

We present a novel symbolic reasoning engine for SQL which can efficiently generate an input $I$ for $n$ queries $P_1, \cdots, P_n$, such that their outputs on $I$ satisfy a given property (expressed in SMT). This is useful in different contexts, such as disproving equivalence of two SQL queries and disambiguating a set of queries. Our first idea is to reason about an under-approximation of each $P_i$ -- that is, a subset of $P_i$'s input-output behaviors. While it makes our approach both semantics-aware and lightweight, this idea alone is incomplete (as a fixed under-approximation might miss some behaviors of interest). Therefore, our second idea is to perform search over an expressive family of under-approximations (which collectively cover all program behaviors of interest), thereby making our approach complete. We have implemented these ideas in a tool, Polygon, and evaluated it on over 30,000 benchmarks across two tasks (namely, SQL equivalence refutation and query disambiguation). Our evaluation results show that Polygon significantly outperforms all prior techniques.

==> figures/fig-gen-mutant.tex <==
In text, we should make it clear that each $\subast$ is a unique subAST even if two share the same string representation. I was thinking to explicitly add a label to each subAST but thought that might be too much. 


We probably don't need rules for BuildAST. Just say we replace each hole $\hole_{\grammarsymbol}$ in $\sketch'$ with $\holemapping[\hole_{\grammarsymbol}]$. Note that while the substituted subASTs are reused, the other AST nodes are fresh new.



\begin{figure}[!t]
\small 
\centering
\[
\begin{array}{c}

(1) \ \ 
\irule{
\begin{array}{c}
\textsc{Match}(\sketch, \subast) = \holemapping 
\\ 
\textsc{BuildAST}(\sketch', \holemapping) = \subast'
\end{array}
}
{
\genkillcondition{\sketch \sketchtosketch \sketch'}{\subast}{\subast'}
}

\ \ \ \ \ \ 

(2) \ \ 
\irule
{
\begin{array}{c}
\subast = \queryop( \subast_1, \mydots, \subast_n) 
\ \ \ \ 
\sketch \rightsquigarrow \sketch' \vdash \subast_i : \subast'_i 
\\ 
\text{fresh} \ \subast' = \queryop( \subast_1, \mydots, \subast_{i-1}, \subast_i', \subast_{i+1}, \mydots, \subast_n)
\end{array}
}
{\genkillcondition{\sketch \sketchtosketch \sketch'}{\subast}{\subast'}}

\end{array}
\]
\caption{Rules for \textnormal{\textsc{GenMutants}}.}
\label{fig:gen-mutant}
\end{figure}



\begin{figure}
\small 
\centering
\[
\begin{array}{cc}

(1) \ \ 
\irule{
\sketch = \queryop ( \sketch_1, \mydots, \sketch_n ) 
\ \ \ \ 
\subast = \queryop ( \subast_1, \mydots, \subast_n ) 
\ \ \ \ 
\matchsubastagainstsketch{\sketch_i}{\subast_i}{\holemapping_i}
}{
\matchsubastagainstsketch{\sketch}{\subast}{ \bigcup_{1 \leq i \leq n} \holemapping_i}
}

\ \ \ \ \ \ 

(2) \ \ 
\irule{

}{
\matchsubastagainstsketch{\hole_{\grammarsymbol}}{\subast}{ \{ \hole_{\grammarsymbol} \mapsto \subast \} }
}

\end{array}
\]

\caption{Rules for \textnormal{\textsc{Match}}.}
\end{figure}




    


\begin{figure}[!t]
\small 
\centering
\[
\begin{array}{c}

\irulelabel
{}
{\vdash \textsc{Match}(e, e) : \emptyset}
{\textrm{(Match1)}}

\irulelabel
{}
{\vdash \textsc{Match}(\hole_e, e) : \set{\hole_e \mapsto e}}
{\textrm{(Match2)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\sketch = \sketch_f(\sketch_1, \ldots, \sketch_n) \quad e = f(e_1, \ldots, e_n) \\
\vdash \textsc{Match}(\sketch_f, f) : \holemapping_f \\
\vdash \textsc{Match}(\sketch_i, e_i) : \holemapping_i \quad 1 \leq i \leq n
\end{array}}
{\vdash \textsc{Match}(\sketch, e) : \holemapping_f \doubleplus \holemapping_1 \doubleplus \ldots \doubleplus \holemapping_n}
{\textrm{(Match3)}}

\\ \ \\

\irulelabel
{}
{\vdash \textsc{BuildAST}(e, \holemapping) : e}
{\textrm{(BuildAST1)}}

\irulelabel
{}
{\vdash \textsc{BuildAST}(\hole_e, \holemapping[\hole_e \mapsto e]) : e}
{\textrm{(BuildAST2)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\sketch = \sketch_f(\sketch_1, \ldots, \sketch_n) \\
\vdash \textsc{BuildAST}(\sketch_f, \holemapping) : f \\
\vdash \textsc{BuildAST}(\sketch_i, \holemapping) : e_i \quad 1 \leq i \leq n \\
e = f(e_1, \ldots, e_n)
\end{array}}
{\vdash \textsc{BuildAST}(\sketch, \holemapping) : e}
{\textrm{(BuildAST3)}}

\\ \ \\

\irulelabel
{\textsc{Match}(\sketch, e) = \holemapping \quad \textsc{BuildAST}(\sketch', \holemapping) = e'}
{\sketch \rightsquigarrow \sketch' \vdash e : e'}
{\textrm{(Root)}}

% \irulelabel
% {\textsc{Match}(\sketch, e) = \bot}
% {\sketch \rightsquigarrow \sketch' \vdash e : \bot}
% {\textrm{(Root2)}}

% \\ \ \\

\irulelabel
{\begin{array}{c}
e = f(e_1, \ldots, e_n) \\
\exists i. ~ 1 \leq i \leq n \quad \sketch \rightsquigarrow \sketch' \vdash e_i : e_i' \\
\text{fresh} ~ e' = f(e_1, \ldots, e_{i-1}, e_i', e_{i+1}, \ldots, e_n)
\end{array}}
{\sketch \rightsquigarrow \sketch' \vdash e : e'}
{\textrm{(Children)}}


% \irulelabel
% {\begin{array}{c}
% e = f(e_1, \ldots, e_n) \\
% \sketch \rightsquigarrow \sketch' \vdash e_i : \bot \quad 1 \leq i \leq n
% \end{array}}
% {\sketch \rightsquigarrow \sketch' \vdash e : \bot}
% {\textrm{(Sub2)}}

% \irulelabel
% {\begin{array}{c}
% e = f(e_1, \ldots, e_n) \\
% \textsc{Match}(\sketch, e) = \holemapping \quad \textsc{BuildAST}(\sketch', \holemapping) = e' \\
% \sketch \rightsquigarrow \sketch' \vdash e_i : S_i \quad 1 \leq i \leq n \\
% S'_i = \set{f(e_1, \ldots, e_{i-1}, e'_i, e_{i+1}, \ldots, e_n) ~|~ e'_i \in S_i}
% \end{array}}
% {\sketch \rightsquigarrow \sketch' \vdash e : \set{e'} \cup S_1' \cup \ldots \cup S_n'}
% {\textrm{(Comp1)}}

% \irulelabel
% {\begin{array}{c}
% e = f(e_1, \ldots, e_n) \\
% \textsc{Match}(\sketch, e) = \bot \\
% \sketch \rightsquigarrow \sketch' \vdash e_i : S_i \quad 1 \leq i \leq n \quad \exists i. ~ S_i \neq \emptyset \\
% S'_i = \set{f(e_1, \ldots, e_{i-1}, e'_i, e_{i+1}, \ldots, e_n) ~|~ e'_i \in S_i}
% \end{array}}
% {\sketch \rightsquigarrow \sketch' \vdash e : S_1' \cup \ldots \cup S_n'}
% {\textrm{(Comp2)}}

\end{array}
\]
\caption{\textsc{GenMutations} rules}
\label{fig:gen-mutant}
\end{figure}






==> figures/fig-mutation-rules.tex <==
\begin{figure}[!t]
\scriptsize
\centering
\[
\begin{array}{c}
\irulelabel
{\begin{array}{c}
\alllogic_1, \alllogic_2 \in \set{\leq, <, =, \neq, >, \geq} \quad
\alllogic_2 \neq \alllogic_1 \\
\end{array}}
{\hole_{E_1} \alllogic_1 \hole_{E_2} \rightsquigarrow \hole_{E_1} \alllogic_2 \hole_{E_2}}
{\text{(Comparison)}}

\\ \ \\

\irulelabel
{\hole_Q \in \set{R, \proj_L(Q)}}
{\hole_Q \rightsquigarrow \text{Distinct}(\hole_Q)}
{\text{(TableDistinct-A)}}

\irulelabel
{\hole_Q \in \set{R, \proj_L(Q)}}
{\text{Distinct}(\hole_Q) \rightsquigarrow \hole_Q}
{\text{(TableDistinct-B)}}


\\ \ \\

\irulelabel
{\begin{array}{c}
\alljoin_1, \alljoin_2 \in \set{\ijoin, \ljoin, \rjoin, \fjoin} \quad
\alljoin_1 \neq \alljoin_2 \\
\end{array}}
{\alljoin_1(\hole_{Q_1}, \hole_{Q_2}, \hole_\phi) \rightsquigarrow \alljoin_2(\hole_{Q_1}, \hole_{Q_2}, \hole_\phi)}
{\text{(JoinType)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\alljoin \in \set{\ijoin, \ljoin, \rjoin, \fjoin}
\end{array}}
{\alljoin_1(\hole_{Q_1}, \hole_{Q_2}, \hole_\phi) \rightsquigarrow \hole_{Q_1}\times \hole_{Q_2}}
{\text{(DropJoinPred)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\mathcal{G}_1, \mathcal{G}_2 \in \set{\text{Count}, \text{Min}, \text{Max}, \text{Sum}, \text{Avg}} \quad
\mathcal{G}_1 \neq \mathcal{G}_2
\\
\end{array}}
{\mathcal{G}_1(\hole_b, \hole_E) \rightsquigarrow \mathcal{G}_2(\hole_b, \hole_E)}
{\text{(AggFun)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\mathcal{G} \in \set{\text{Count}, \text{Sum}, \text{Avg}}
\\
b_1, b_2 \in \set{\top, \bot} \quad
b_1 \neq b_2
\end{array}}
{\mathcal{G}(\hole_{b_1}, \hole_E) \rightsquigarrow \mathcal{G}(\hole_{b_2}, \hole_E)}
{\text{(AggFunDistinct)}}

\\ \ \\

\irulelabel
{}
{\text{Count}(\bot, \hole_E) \rightsquigarrow \text{Count}(\bot, *)}
{\text{(CountAttrToStar)}}

\\ \ \\

\irulelabel
{}
{\hole_{\phi_1} \land \hole_{\phi_2} \rightsquigarrow \hole_{\phi_1} \lor \hole_{\phi_2}}
{\text{(BoolOp-A)}}

\irulelabel
{}
{\hole_{\phi_1} \lor \hole_{\phi_2} \rightsquigarrow \hole_{\phi_1} \land \hole_{\phi_2}}
{\text{(BoolOp-B)}}

\\ \ \\

\irulelabel
{}
{\hole_{\phi_1} \land \hole_{\phi_2} \rightsquigarrow \top \land \hole_{\phi_2}}
{\text{(ConjunctDropClause-A)}}

\irulelabel
{}
{\hole_{\phi_1} \land \hole_{\phi_2} \rightsquigarrow \hole_{\phi_1} \land \top}
{\text{(ConjunctDropClause-B)}}

\\ \ \\

\irulelabel
{}
{\hole_{\phi_1} \lor \hole_{\phi_2} \rightsquigarrow \bot \lor \hole_{\phi_2}}
{\text{(DisjunctDropClause-A)}}

\irulelabel
{}
{\hole_{\phi_1} \lor \hole_{\phi_2} \rightsquigarrow \hole_{\phi_1} \lor \bot}
{\text{(DisjunctDropClause-B)}}

\\ \ \\

\irulelabel
{}
{\filter_{\hole_\phi}(\hole_Q) \rightsquigarrow \filter_{\top}(\hole_Q)}
{\text{(DropFilter)}}

\\ \ \\

\irulelabel
{}
{\text{GroupBy}(\hole_Q, \hole_{\vec{E}}, \hole_L, \hole_\phi) \rightsquigarrow \text{GroupBy}(\hole_Q, \hole_{\vec{E}}, \hole_L, \top)}
{\text{(DropHaving)}}

\\ \ \\

\irulelabel
{}
{\hole_{Q_1} \cup \hole_{Q_2} \rightsquigarrow \hole_{Q_1} \uplus \hole_{Q_2}}
{\text{(UnionDistinct-A)}}

\irulelabel
{}
{\hole_{Q_1} \uplus \hole_{Q_2} \rightsquigarrow \hole_{Q_1} \cup \hole_{Q_2}}
{\text{(UnionDistinct-B)}}

\\ \ \\

\irulelabel
{}
{\text{OrderBy}(\hole_Q, \hole_{\vec{E}}, \hole_b) \rightsquigarrow \text{OrderBy}(\hole_Q, \top, \hole_b)}
{\text{(DropOrderBy)}}


\end{array}
\]
\caption{Mutation rules.}
\label{fig:mutation-rules}
\end{figure}


==> figures/fig-vec-encoding.tex <==
\begin{figure}[!t]
\scriptsize
\centering
\[
\begin{array}{c}

\irulelabel
{\begin{array}{c}

\underapprox_i \neq \unknown
\end{array}}
{ \encodechoice \leadsto \encvector_i = \underapprox_i}
{(\textsc{Known})}


\irulelabel
{\begin{array}{c}

\underapprox_i = \unknown \quad
\underapprox \in \mathbb{D}^n \quad
\mathbb{D} = \set{c_1, \cdots, c_m, \unknown}
\end{array}}
{ \encodechoice(\astnode, \underapprox) \leadsto \encvector_i = \underapprox_i }
{(\textsc{Unknown})}


\end{array}
\]

\caption{Encoding choices of under-approximations.}
\label{fig:encode-ua-choice}
\end{figure}


==> stale/stale-fig-under-semantics.tex <==
\begin{figure}[!t]
\scriptsize
\centering
\[
\begin{array}{c}

\irulelabel
{\begin{array}{c}
\neg \text{hasAgg(L)} \quad
\relation = [\tuple_1, \ldots, \tuple_n] \quad
\relation' = [\tuple'_{1}, \ldots, \tuple'_n] \quad
L = [a_1', \ldots, a_{l}'] \quad
\undervector \in \bdom^n \\
\formula = \land_{i=1}^n (
(\undervector_i \to \neg \del(\tuple_i) \land \land_{j=1}^{l} 
    \denot{t'_i.a'_j} = \denot{t_i.a'_j} \land \neg \del(\tuple_i'))
\land
(\neg \undervector_i \to \del(\tuple_i) \land \del(\tuple_i'))
)\\
\end{array}}
{\undervector \vdash \proj_L(\relation) \Downarrow \relation' \leadsto \formula}
{\text{(Project)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\relation = [\tuple_1, \ldots, \tuple_n] \quad
\relation' = [\tuple'_{1}, \ldots, \tuple'_n] \quad
\undervector \in \bdom^n \\
\formula = \land_{i=1}^n (
(\undervector_i \to \neg \del(\tuple_i) \land \denot{\phi}_{\tuple_i} \land \neg \del(\tuple_i') \land \tuple_{i}' = \tuple_{i})
\land
(\neg \undervector_i \to ( (\del(\tuple_i) \lor (\neg \del(\tuple_i) \land \neg \denot{\phi}_{\tuple_i}) ) \land \del(\tuple_i'))
)
)\\
\end{array}}
{\undervector \vdash \filter_\phi(\relation) \Downarrow \relation' \leadsto \formula}
{\text{(Filter)}}

\\ \ \\



\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1,1}, \ldots, \tuple''_{n,m}] \quad
\undervector \in \bdom^{n \times m} \\

\text{Attrs}(\relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\relation_2) = [a'_1, \ldots, a'_{q}] \\

\formula = \land_{i=1}^n \land_{j=1}^m (
(\undervector_{i,j} \to \neg \del(t_i) \land \neg \del(t'_j) \land \land_{k=1}^{p} \denot{t''_{i,j}.a_{k}} = \denot{t_i.a_{k}} \land \land_{k=1}^{q} \denot{t''_{i,j}.a_{k}'} = \denot{t'_{j}.a_{k}'}) \\
\land (\neg \undervector_{i,j} \to (\del(t_i) \lor \del(t'_j)) \land \del(t''_{i,j}))
)

\end{array}}
{\undervector \vdash \relation_1 \times \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(Product)}}


\\ \ \\


\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1,1}, \ldots, \tuple''_{n,m}] \quad
\undervector \in \bdom^{n \times m} \\

\text{Attrs}(\relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\relation_2) = [a'_1, \ldots, a'_{q}] \\

\formula = \land_{i=1}^n \land_{j=1}^m (
\land_{k=1}^{p} \denot{t''_{i,j}.a_{k}} = \denot{t_i.a_{k}} \land \land_{k=1}^{q} \denot{t''_{i,j}.a_{k}'} = \denot{t'_{j}.a_{k}'} 
\land (\undervector_{i,j} \to \neg \del(t_i) \land \denot{\phi}_{\tuple''_{i,j}} \land \neg \del(t'_j)) \\
\land (\neg \undervector_{i,j} \to (\del(t_i) \lor \del(t'_j) \lor (\neg \del(t_i) \land \neg \del(t'_j) \land \neg \denot{\phi}_{\tuple''_{i,j}})) \land \del(t''_{i,j}))
)

\end{array}}
{\undervector \vdash \relation_1 \ijoin_\phi \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(InnerJoin)}}


\\ \ \\


\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1,1}, \ldots, \tuple''_{n,m}, \tuple''_{1,m+1}, \ldots, \tuple''_{n,m+1}] \quad
\undervector \in \bdom^{n \times m} \\

\text{Attrs}(\relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\relation_2) = [a'_1, \ldots, a'_{q}] \\

\formula = \land_{i=1}^n \land_{j=1}^m (
\land_{k=1}^{p} \denot{t''_{i,j}.a_{k}} = \denot{t_i.a_{k}} \land \land_{k=1}^{q} \denot{t''_{i,j}.a_{k}'} = \denot{t'_{j}.a_{k}'}

\land (\undervector_{i,j} \to \neg \del(t_i) \land \denot{\phi}_{\tuple''_{i,j}} \land \neg \del(t'_j)) \\
\land (\neg \undervector_{i,j} \to (\del(t_i) \lor \del(t'_j) \lor (\neg \del(t_i) \land \neg \del(t'_j) \land \neg \denot{\phi}_{\tuple''_{i,j}})) \land \del(t''_{i,j}))

) \\

\land \land_{i=1}^n( \land_{k=1}^p \denot{t''_{i,m+1}.a_{k}} = \denot{t_i.a_{k}} \land \land_{k=1}^q \denot{t''_{i,m+1}.a'_{k}} = \nullv \land (\neg \del(\tuple_i) \land \land_j^m \neg \undervector_{i,j}) \leftrightarrow \neg \del(\tuple''_{i, m+1}) )

\end{array}}
{\undervector \vdash \relation_1 \ljoin_\phi \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(LeftJoin)}}


\\ \ \\


\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1,1}, \ldots, \tuple''_{n,m}, \tuple''_{n+1,1}, \ldots, \tuple''_{n+1,m}] \quad
\undervector \in \bdom^{n \times m} \\

\text{Attrs}(\relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\relation_2) = [a'_1, \ldots, a'_{q}] \\

\formula = \land_{i=1}^n \land_{j=1}^m (
\land_{k=1}^{p} \denot{t''_{i,j}.a_{k}} = \denot{t_i.a_{k}} \land \land_{k=1}^{q} \denot{t''_{i,j}.a_{k}'} = \denot{t'_{j}.a_{k}'}

\land (\undervector_{i,j} \to \neg \del(t_i) \land \denot{\phi}_{\tuple''_{i,j}} \land \neg \del(t'_j)) \\
\land (\neg \undervector_{i,j} \to (\del(t_i) \lor \del(t'_j) \lor (\neg \del(t_i) \land \neg \del(t'_j) \land \neg \denot{\phi}_{\tuple''_{i,j}})) \land \del(t''_{i,j}))

) \\

\land \land_{j=1}^m( \land_{k=1}^p \denot{t''_{n+1,j}.a_{k}} = \nullv \land \land_{k=1}^q \denot{t''_{n+1,j}.a'_{k}} = \denot{\tuple'_j.a'_k} \land (\neg \del(\tuple'_j) \land \land_i^n \neg \undervector_{i,j}) \leftrightarrow \neg \del(\tuple''_{n+1, j}) )

\end{array}}
{\undervector \vdash \relation_1 \rjoin_\phi \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(RightJoin)}}


\\ \ \\


\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1,1}, \ldots, \tuple''_{n,m}, \tuple''_{1,m+1}, \ldots, \tuple''_{n,m+1}, \tuple''_{n+1,1}, \ldots, \tuple''_{n+1,m}] \quad
\undervector \in \bdom^{n \times m} \\

\text{Attrs}(\relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\relation_2) = [a'_1, \ldots, a'_{q}] \\

\formula = \land_{i=1}^n \land_{j=1}^m (
\land_{k=1}^{p} \denot{t''_{i,j}.a_{k}} = \denot{t_i.a_{k}} \land \land_{k=1}^{q} \denot{t''_{i,j}.a_{k}'} = \denot{t'_{j}.a_{k}'}

\land (\undervector_{i,j} \to \neg \del(t_i) \land \denot{\phi}_{\tuple''_{i,j}} \land \neg \del(t'_j)) \\
\land (\neg \undervector_{i,j} \to (\del(t_i) \lor \del(t'_j) \lor (\neg \del(t_i) \land \neg \del(t'_j) \land \neg \denot{\phi}_{\tuple''_{i,j}})) \land \del(t''_{i,j}))

) \\

\land \land_{i=1}^n( \land_{k=1}^p \denot{t''_{i,m+1}.a_{k}} = \denot{t_i.a_{k}} \land \land_{k=1}^q \denot{t''_{i,m+1}.a'_{k}} = \nullv \land (\neg \del(\tuple_i) \land \land_j^m \neg \undervector_{i,j}) \leftrightarrow \neg \del(\tuple''_{i, m+1}) ) \\

\land \land_{j=1}^m( \land_{k=1}^p \denot{t''_{n+1,j}.a_{k}} = \nullv \land \land_{k=1}^q \denot{t''_{n+1,j}.a'_{k}} = \denot{\tuple'_j.a'_k} \land (\neg \del(\tuple'_j) \land \land_i^n \neg \undervector_{i,j}) \leftrightarrow \neg \del(\tuple''_{n+1, j}) )

\end{array}}
{\undervector \vdash \relation_1 \ljoin_\phi \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(FullJoin)}}


\\ \ \\

\irulelabel
{\begin{array}{c}
\relation = [\tuple_1, \ldots, \tuple_n] \quad
\relation' = [\tuple'_{1}, \ldots, \tuple'_n] \quad
\undervector \in \bdom^n \\
\formula = \land_{i=1}^n (
(\undervector_i \to \neg \del(\tuple_i) \land \land_{j=1}^{i-1} t_i \neq t_j \land \neg \del(\tuple_i') \land \tuple_{i}' = \tuple_{i})
\land
(\neg \undervector_i \to ( (\del(\tuple_i) \lor (\neg \del(\tuple_i) \land \lor_{j=1}^{i-1} t_i = t_j) ) \land \del(\tuple_i'))
)
)
\end{array}}
{\undervector \vdash \text{Distinct}(\relation) \Downarrow \relation' \leadsto \formula}
{\text{(Distinct)}}


\\ \ \\

\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_{1}, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1}, \ldots, \tuple''_{n+m}] \quad
\undervector \in \bdom^{n+m} \\
\formula = \land_{i=1}^n (
(\undervector_i \to \neg \del(\tuple_i) \land \neg \del(\tuple''_i) \land \tuple''_{i} = \tuple_{i})
\land
(\neg \undervector_i \to ( \del(\tuple_i) \land \del(\tuple''_i) ))
) \\
\land
\land_{i=n+1}^{n+m} (
(\undervector_i \to \neg \del(\tuple'_{i-n}) \land \neg \del(\tuple''_i) \land \tuple''_{i} = \tuple'_{i-n})
\land
(\neg \undervector_i \to ( \del(\tuple'_{i-n}) \land \del(\tuple''_i) ))
)
\end{array}}
{\undervector \vdash \relation_1 \uplus \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(UnionAll)}}


\\ \ \\

\irulelabel
{\begin{array}{c}

\undervector \vdash \text{Distinct}(\relation_1 \uplus \relation_2) \Downarrow \relation' \leadsto \formula
\end{array}}
{\undervector \vdash \relation_1 \cup \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(Union)}}


\end{array}
\]
\caption{Underapproximate semantics.}
\label{fig:under-semantics}
\end{figure}


==> stale/stale2-fig-under-semantics-b.tex <==
\begin{figure}[!t]
\scriptsize
\centering
\[
\begin{array}{c}

\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1}, \ldots, \tuple''_K] \\
\text{Attrs}(\schema, \relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\schema, \relation_2) = [a'_1, \ldots, a'_{q}] \\

\text{fresh} ~ c_{i, j} \quad 1 \leq i \leq n, 1 \leq j \leq m \\

% b_i = true means the ith tuple in the left table isn't joined to any tuple in the right table
\formula = 0 \leq \size(\relation_1) \leq n \land 0 \leq \size(\relation_2) \leq m \land (p_{i,j} \leftrightarrow \denot{\phi}_{\schema, \symdb, [c_{i,j}]}) \land 
(b_j \leftrightarrow \land_{i=1}^n p_{i,j}=\bot) \land
\\

\land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [c_{i, j}]} \leftrightarrow \denot{a_{k}}_{\schema, \symdb, [\tuple_{i}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [c_{i, j}]} \leftrightarrow \denot{a_{k}'}_{\schema,\symdb,[\tuple_{j}']} \land \\

\bigland\limits_{u=0}^{n} \bigland\limits_{v=0}^{m} \size(\relation_1) = u \land \size(\relation_2) = v \to \size(\relation') = \sum\limits_{j=1}^{v} (\indicator(b_j) + \sum\limits_{i=1}^{u} \indicator(p_{i, j})) \land \\

\bigland\limits_{\size(\relation') \leq \underparam} N = (\size(\relation')-\sum\limits_{j=1}^{v} \indicator(n_j)) \land \land_{x=1}^{N} \texttt{findNthTrueIndex}(x) = (l, r) \to \tuple''_x = c_{l,r} \land \\

\bigland\limits_{x=1}^{\sum\limits_{j=1}^{v} \indicator(b_j)} \land_{j=1}^v b_j \to \land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [\tuple''_{N + x}]} = \nullv \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [\tuple''_{N + x}]} = \denot{a_{k}}_{\schema, \symdb, [\tuple_{j}]}

\end{array}}
{\schema, \symdb \vdash \rjoin(\relation_1, \relation_2, \phi) \Downarrow \relation' \leadsto \formula}
{\text{(RightJoin)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1}, \ldots, \tuple''_K] \\
\text{Attrs}(\schema, \relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\schema, \relation_2) = [a'_1, \ldots, a'_{q}] \\

\text{fresh} ~ c_{i, j} \quad 1 \leq i \leq n, 1 \leq j \leq m \\

% b_i = true means the ith tuple in the left table isn't joined to any tuple in the right table
\formula = 0 \leq \size(\relation_1) \leq n \land 0 \leq \size(\relation_2) \leq m \land (p_{i,j} \leftrightarrow \denot{\phi}_{\schema, \symdb, [c_{i,j}]}) \land 
(b_i \leftrightarrow \land_{j=1}^m p_{i,j}=\bot) \land (b'_j \leftrightarrow \land_{i=1}^n p_{i,j}=\bot) \land
\\

\land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [c_{i, j}]} \leftrightarrow \denot{a_{k}}_{\schema, \symdb, [\tuple_{i}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [c_{i, j}]} \leftrightarrow \denot{a_{k}'}_{\schema,\symdb,[\tuple_{j}']} \land \\

\bigland\limits_{u=0}^{n} \bigland\limits_{v=0}^{m} \size(\relation_1) = u \land \size(\relation_2) = v \to \size(\relation') = \sum\limits_{i=1}^{u} (\indicator(b_i) + \sum\limits_{j=1}^{v} \indicator(p_{i, j})) + \sum\limits_{j=1}^{v} \indicator(b_j) \land \\

\bigland\limits_{\size(\relation') \leq \underparam} N = (\size(\relation') - \sum\limits_{i=1}^{u} \indicator(b_i) -\sum\limits_{j=1}^{v} \indicator(b_j)) \land \land_{x=1}^{N} \texttt{findNthTrueIndex}(x) = (l, r) \to \tuple''_x = c_{l,r} \land \\

\bigland\limits_{x=1}^{\sum\limits_{i=1}^{u} \indicator(b_i)} \land_{i=1}^u b_i \to \land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [\tuple''_{N + x}]} = \denot{a_{k}}_{\schema, \symdb, [\tuple_{i}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [\tuple''_{N + x}]} = \nullv \ \land \\

\bigland\limits_{x=1}^{\sum\limits_{j=1}^{v} \indicator(b_j)} \land_{j=1}^v b_j \to \land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [\tuple''_{N + \sum\limits_{i=1}^{u} \indicator(b_i) + x}]} = \nullv \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [\tuple''_{N + \sum\limits_{i=1}^{u} \indicator(b_i) + x}]} = \denot{a_{k}}_{\schema, \symdb, [\tuple_{j}]}

\end{array}}
{\schema, \symdb \vdash \fjoin(\relation_1, \relation_2, \phi) \Downarrow \relation \leadsto \formula}
{\text{(FullJoin)}}

\\ \ \\

\irulelabel
{\begin{array}{c}

\relation = [\tuple_1, \ldots, \tuple_n] \quad
\relation' = [\tuple'_{1}, \ldots, \tuple'_\underparam] \quad
L = [a'_1, \ldots, a'_l] \\

\formula = 0 \leq \size(\relation) \leq n \land \bigland\limits_{u=0}^{n} \size(\relation) = u \to \grouping(\relation, i, \group) \leftrightarrow \bigland\limits_{e \in \vec{E}} \land_{i=1}^u \land_{i'=1}^u \denot{e}_{\schema, \symdb, [i]} = \denot{e}_{\schema, \symdb, [i']} \to \\
\bigland\limits_{N=0}^\underparam \land_{i=1}^u \exists \group. ~ (\grouping(\relation, i, \group) \land 1 \leq g \leq \underparam \to (\land_{\group'=1}^\underparam \group' \neq \group \to \neg \grouping(\relation, i, \group'))) \land p_g \leftrightarrow \denot{\phi}_{\schema, \symdb, \grouping^{-1}(\relation, g)} \to \\

\size(\relation') = \sum_{g=1}^N \indicator(p_g) \land \bigland\limits_{x=1}^{\size(\relation')} \exists g'. ~ (p_{g'} = \top \land \sum_{g=1}^{g'} \indicator(g_i = \top) = x) \to \land_{k=1}^l \denot{a'_l}_{\schema, \symdb, [t'_x]} = \denot{a'_l}_{\schema, \symdb, \grouping^{-1}(\relation, g')}

\end{array}}
{\schema, \symdb \vdash \text{GroupBy}(\relation, \vec{E}, L, \phi) \Downarrow \relation' \leadsto\formula}
{\text{(GroupBy)}}

\\ \ \\

\irulelabel
{\begin{array}{c}

\relation = [\tuple_1, \ldots, \tuple_n] \quad
\relation' = [\tuple'_{1}, \ldots, \tuple'_n] \\

% this means the ith tuple in the input table is ranked xth
\Psi_{n} = \set{\bigland\limits_{i=1}^n (\exists x. (\text{rankedNth}(i, x, \vec{E}, b) \land \nexists i'. \text{rankedNth}(i', x, \vec{E}, b)) \to t'_x = t_i)} \quad 1 \leq |\Psi_n| \leq \underparam \\

\Psi'_{n} = \set{\bigland\limits_{i=1}^n (\exists x. (\text{rankedNth}(i, x, \vec{E}, b) \land \nexists i'. \text{rankedNth}(i', x, \vec{E}, b)))} \quad 1 \leq |\Psi'_n| \leq \underparam \\


\formula = 0 \leq \size(\relation) \leq n \land \bigland\limits_{u=0}^{n} \size(\relation) = u \to \size(\relation') = u \land \bigland\limits_{\psi_i \in \Psi_{u}} \psi_i \land \biglor\limits_{\psi'_i \in \Psi'_{u}} \psi'_i
 \\

\end{array}}
{\schema, \symdb, \underparam \vdash \text{OrderBy}(\relation, \vec{E}, b) \Downarrow \relation' \leadsto\formula}
{\text{(OrderBy)}}

\end{array}
\]
\caption{Underapproximate semantics (cont.)}
\label{fig:under-semantics-b}
\end{figure}


==> stale/stale2-fig-under-semantics.tex <==
\begin{figure}[!t]
\scriptsize
\centering
\[
\begin{array}{c}

% \irulelabel
% {R \in \text{Dom}(\symdb)}
% {\schema, \symdb, \param \vdash R \leadsto \top}
% {\text{(Relation)}}

% \irulelabel
% {\begin{array}{c}
% \schema, \symdb, \param \vdash Q \leadsto \formula
% \end{array}}
% {\schema, \symdb, \param \vdash \rename_X(Q) \leadsto \formula}
% {\text{(Rename)}}

% \\ \ \\

% \irulelabel
% {\begin{array}{c}
% \neg \text{hasAgg}(L) \\
% \symdb \vdash Q \hookrightarrow R_1 \quad
% R_1 = [t_1, \ldots, t_n] \quad
% \schema, \symdb, \param \vdash Q \leadsto \formula_1 \\

% \schema \vdash \proj_L(Q) : [a'_1, \ldots, a'_{l}] \quad
% \symdb \vdash \proj_L(Q)  \hookrightarrow R \quad
% R = [t'_{1}, \ldots, t'_{n}] \\

% \formula = \bigland\limits_{u=0}^{n} \size(R_1) = u \to
% \size(R) = u \land \bigland\limits_{i=1}^{u} (\land_{p=1}^l \denot{a'_p}_{\schema, \symdb, [t_i']} = \denot{a'_p}_{\schema, \symdb, [t_i]})

% \end{array}}
% {\schema, \symdb, \param \vdash \proj_L(Q) \leadsto \formula_1 \land \formula}
% {\text{(Projection)}}

% \\ \ \\

% \irulelabel
% {\begin{array}{c}
% \text{hasAgg}(L) \\
% \symdb \vdash Q \hookrightarrow R_1 \quad
% R_1 = [t_1, \ldots, t_n] \quad
% \schema, \symdb, \param \vdash Q \leadsto \formula_1 \\

% \schema \vdash \proj_L(Q) : [a'_1, \ldots, a'_{l}] \quad
% \symdb \vdash \proj_L(Q)  \hookrightarrow R \quad
% R = [t'_{1}, \ldots, t'_{n}] \\

% \formula = \bigland\limits_{u=0}^{n} \size(R_1) = u \to
% \size(R) = 1 \land \land_{p=1}^l \denot{a'_p}_{\schema, \symdb, [t_1']} = \denot{a'_p}_{\schema, \symdb, [t_1, \ldots, t_u]}

% \end{array}}
% {\schema, \symdb, \param \vdash \proj_L(Q) \leadsto \formula_1 \land \formula}
% {\text{(AggProjection)}}

\\ \ \\

\irulelabel
{\begin{array}{c}

%\param = \param_1 \uplus [\filter_\phi(Q) \mapsto K] \\

%\text{Attrs}(\schema, Q) = [a_1, \ldots, a_{p}] \quad
%\text{Tuples}(\symdb, Q) = R_1 \quad
\relation = [\tuple_1, \ldots, \tuple_n] \quad
%\schema, \symdb, \param_1 \vdash Q \leadsto \formula_1 \\

%\text{Tuples}(\symdb, \filter_\phi(Q)) = R \quad
\relation' = [\tuple'_{1}, \ldots, \tuple'_\underparam] \quad

\undermapping[v] = \undervector \\

\formula = \land_{i=1}^n (
(\undervector_i = \top \to \neg \del(\tuple_i) \land \denot{\phi}_{\schema, \symdb, [t_i]} = \top \land \neg \del(\tuple_i') \land \tuple_{i}' = \tuple_{i})
\land
(\undervector_i = \bot \to \neg (\neg \del(\tuple_i) \land \denot{\phi}_{\schema, \symdb, [t_i]} = \top) \land \del(\tuple_i'))
)\\


% \formula = 0 \leq \size(\relation) \leq n \land \bigland\limits_{u=0}^{n} \size(\relation) = u \land (p_i \leftrightarrow \denot{\phi}_{\schema, \symdb, [\tuple_i]}) \to \\
% \size(\relation') = \sum\limits_{i=1}^{u}\indicator(p_i) \land ( \biglor\limits_{\size(\relation') \leq \underparam} \land_{i=1}^u p_i ) \land \bigland\limits_{\size(\relation') \leq \underparam} (\land_{x=1}^{\size(\relation')} \exists i'. ~ (p_{i'} = \top \land \sum_{i=1}^{i'} \indicator(p_i = \top) = x) \to \tuple'_x = \tuple_{i'})\\
% \land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [t_x']} = \denot{a_{k}}_{\schema, \symdb, [t_{i'}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [t_x']} = \denot{a_{k}'}_{\schema,\symdb,[t_{i'}]} \\[1.2em]

% \formula_{\text{UA}} = \bigvee\limits_{u=0}^{n} \size(R_1) = u \land (p_i \leftrightarrow \denot{\phi}_{\schema, \symdb, [t_i]}) \to \\
% \size(R) = \sum\limits_{i=1}^{u}\indicator(p_i) \land \bigland\limits_{\size(R) \leq K} \land_{i=1}^u p_i

\end{array}}
{\schema, \symdb, \undermapping \vdash v : \filter_\phi(\relation) \Downarrow \relation' \leadsto \formula}
{\text{(Filter)}}

\\ \ \\

\irulelabel
{\begin{array}{c}

\relation = [\tuple_1, \ldots, \tuple_n] \quad \quad
\relation' = [\tuple'_1, \ldots, \tuple'_\underparam] \\

% p_i being true means the ith tuple is unique
\formula = 0 \leq \size(\relation) \leq n \land \bigland\limits_{u=0}^{n} \size(\relation) = u \land (p_i \leftrightarrow \land_{j=1}^{u} (i \neq j \to \tuple_i \neq \tuple_j)) \to \\

\size(\relation') = \sum\limits_{i=1}^{u}\indicator(p_i) \land ( \biglor\limits_{\size(\relation') \leq \underparam} \land_{i=1}^u p_i ) \land \bigland\limits_{\size(\relation') \leq \underparam} (\land_{x=1}^{\size(\relation')} \exists i'. ~ (p_{i'} = \top \land \sum_{i=1}^{i'} \indicator(p_i = \top) = x) \to \tuple'_x = \tuple_{i'}) \\
% \land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [t_x']} = \denot{a_{k}}_{\schema, \symdb, [t_{i'}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [t_x']} = \denot{a_{k}'}_{\schema,\symdb,[t_{i'}]} \\[1.2em]

% \formula_{\text{UA}} = \bigvee\limits_{u=0}^{n} \size(R_1) = u \land (p_i \leftrightarrow \land_{j=1}^{u} (i \neq j \to t_i \neq t_j)) \to \\
% \size(R) = \sum\limits_{i=1}^{u}\indicator(p_i) \land \bigland\limits_{\size(R) \leq K} \land_{i=1}^u p_i

\end{array}}
{\schema, \symdb \vdash \text{Distinct}(\relation) \Downarrow \relation' \leadsto \formula}
{\text{(Distinct)}}

\\ \ \\

\irulelabel
{\begin{array}{c}

\schema, \symdb \vdash \text{Distinct}(\relation_1 \uplus \relation_2) \Downarrow \relation' \leadsto \formula
\end{array}}
{\schema, \symdb \vdash \relation_1 \cup \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(Union)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_1, \ldots, \tuple''_{\underparam}] \\

\formula = \biglor\limits_{u=0}^{n} \biglor\limits_{v=0}^{m} \size(\relation_1) = u \land \size(\relation_2) = v \land 0 \leq \size(\relation_1)+\size(\relation_2) \leq \underparam \land \\ \bigland\limits_{u=0}^{n} \bigland\limits_{v=0}^{m} \size(\relation_1) = u \land \size(\relation_2) = v \to
\size(\relation') = u + v \land \land_{i=1}^u \tuple''_i = \tuple_i \land \land_{i=1}^v \tuple''_{u+i} = \tuple'_i \\
\end{array}}
{\schema, \symdb \vdash \relation_1 \uplus \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(UnionAll)}}


\\ \ \\

\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1}, \ldots, \tuple''_\underparam] \\
\text{Attrs}(\schema, \relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\schema, \relation_2) = [a'_1, \ldots, a'_{q}] \\

\formula = \biglor\limits_{u=0}^{n} \biglor\limits_{v=0}^{m} \size(\relation_1) = u \land \size(\relation_2) = v \land 0 \leq \size(\relation_1) \times \size(\relation_2) \leq \underparam \land \bigland\limits_{u=0}^{n} \bigland\limits_{v=0}^{m} \size(\relation_1) = u \land \size(\relation_2) = v \to \\
\size(\relation') = uv \land \bigland\limits_{i=1}^u \bigland\limits_{j=1}^v \land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [t''_{(i-1) \cdot v + j}]} = \denot{a_{k}}_{\schema, \symdb, [t_{i}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [t''_{(i-1) \cdot v + j}]} = \denot{a_{k}'}_{\schema,\symdb,[t'_{j}]} \\

\end{array}}
{\schema, \symdb \vdash \relation_1 \times \relation_2 \Downarrow \relation' \leadsto \formula}
{\text{(Product)}}

\\ \ \\


\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1}, \ldots, \tuple''_\underparam] \\
\text{Attrs}(\schema, \relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\schema, \relation_2) = [a'_1, \ldots, a'_{q}] \\

\text{fresh} ~ c_{i, j} \quad 1 \leq i \leq n \quad 1 \leq j \leq m \\

\formula_1 = 0 \leq \size(\relation_1) \leq n \land 0 \leq \size(\relation_2) \leq m \land (p_{i,j} \leftrightarrow \denot{\phi}_{\schema, \symdb, [c_{i,j}]}) \land \\

\land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [c_{i, j}]} \leftrightarrow \denot{a_{k}}_{\schema, \symdb, [\tuple_{i}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [c_{i, j}]} \leftrightarrow \denot{a_{k}'}_{\schema,\symdb,[\tuple_{j}']} \land \\

% Enumerate all tuple pairs (power set)
% {(1, 1), (1, 2), (2, 1), (2, 2)}
% p_{1,1}, p_{1,2}, p_{2,1}, p_{2,2}
% p_{1,1}, ~p_{1,2}, p_{2,1}, ~p_{2,2}
% ...
% and each tuple pair may satisfy the join condition or not
% for example, (⊤, ⊤, ⊤, ⊤) means all four pairs satisfy the
% join condition, and (⊥, ⊥, ⊥, ⊤) means only the fourth pair
% satisfies the condition
% Therefore, we also need to enumerate all cases where each
% tuple pair is satisfied or not -- denoted by p_{i,j}
% \bigvee\limits_{p_{i, j} \in \set{\top, \bot}, 1 \leq i \leq u, 1 \leq j \leq v} \land_{i=1}^u \land_{j=1}^v p_{i, j} \to \\


% limit that there may only be up to K p_{i, j} that is ⊤
% for each p_{i, j}, we evaluate the join condition accordingly
% \bigland\limits_{\sum_{i=1}^{u}\sum_{j=1}^{v}\indicator(p_{i, j}) \leq K}(\land_{i=1}^u \land_{j=1}^v p_{i, j} = \top \to \denot{\phi}_{\schema, \symdb, [t_{\todo{i,j}}]} \land p_{i, j} = \bot \to \neg \denot{\phi}_{\schema, \symdb, [t_{\todo{i,j}}]} ) \to \\
\Psi_{n, m} = \bigland\limits_{u=0}^{n} \bigland\limits_{v=0}^{m} \size(\relation_1) = u \land \size(\relation_2) = v \to \size(\relation') = \sum\limits_{i=1}^{u}\sum\limits_{j=1}^{v}\indicator(p_{i, j}) \land \\

\bigland\limits_{\size(\relation') \leq K} 

% o is the output size
% x is the new tuple id in the output table
% xth tuple in the output table corresponds to the xth tuple pair
% that p_{i,j} = ⊤.  This means before xth tuple, there exist
% \(x - 1) tuples that p_{i,j} = ⊤.

% p_{1,1}, ~p_{1,2}, p_{2,1}, ~p_{2,2}
% x = 1 -> p_{1,1}
% t_1'' = concat(t_1, t_1')
% t_2'' = concat(t_2, t_1')
% findNthTrueIndex(x) = (l, r) /\ t''_x = concat(t_l, t_r')
% x = 2 -> p_{2,1}
% \bigland\limits_{1 \leq x \leq \size(R)} \exists l, r. ~ (p_{l,r} = \top \land \sum_{i=1}^l\sum_{j=1}^r \indicator(p_{l, r} = \top) = x-1) \to \\
\land_{x=1}^{\size(R')} \texttt{findNthTrueIndex}(l, r, x) \to

% map all attributes in previous tuples to the new concatenated tuple
% \land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [t_x'']} = \denot{a_{k}}_{\schema, \symdb, [t_{l}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [t_x'']} = \denot{a_{k}'}_{\schema,\symdb,[t_{r}']} \\
\tuple''_x = c_{l,r}

\quad 1 \leq |\Psi_{n, m}| \leq \underbranchparam \\

\formula_2 = \land_{u=0}^{n} \land_{v=n}^{m} \land_{\psi \in \Psi_{n, m}} \psi

\end{array}}
{\schema, \symdb, \underbranchparam \vdash ~ \ijoin(\relation_1, \relation_2, \phi) \Downarrow \relation' \leadsto \formula_1 \land \formula_2}
{\text{(InnerJoin)}}

\\ \ \\

\irulelabel
{\begin{array}{c}
\relation_1 = [\tuple_1, \ldots, \tuple_n] \quad
\relation_2 = [\tuple'_1, \ldots, \tuple'_m] \quad
\relation' = [\tuple''_{1}, \ldots, \tuple''_\underparam] \\
\text{Attrs}(\schema, \relation_1) = [a_1, \ldots, a_{p}] \quad
\text{Attrs}(\schema, \relation_2) = [a'_1, \ldots, a'_{q}] \\

\text{fresh} ~ c_{i, j} \quad 1 \leq i \leq n \quad 1 \leq j \leq m \\

% b_i = true means the ith tuple in the left table isn't joined to any tuple in the right table
\formula = 0 \leq \size(\relation_1) \leq n \land 0 \leq \size(\relation_2) \leq m \land (p_{i,j} \leftrightarrow \denot{\phi}_{\schema, \symdb, [c_{i,j}]}) \land 
(b_i \leftrightarrow \land_{j=1}^m p_{i,j}=\bot) \land
\\

\land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [c_{i, j}]} \leftrightarrow \denot{a_{k}}_{\schema, \symdb, [\tuple_{i}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [c_{i, j}]} \leftrightarrow \denot{a_{k}'}_{\schema,\symdb,[\tuple_{j}']} \land \\

\bigland\limits_{u=0}^{n} \bigland\limits_{v=0}^{m} \size(\relation_1) = u \land \size(\relation_2) = v \to \size(\relation') = \sum\limits_{i=1}^{u} (\indicator(b_i) + \sum\limits_{j=1}^{v} \indicator(p_{i, j})) \land \\

\bigland\limits_{\size(\relation') \leq \underparam} N = (\size(\relation')-\sum\limits_{i=1}^{u} \indicator(b_i)) \land \land_{x=1}^{N} \texttt{findNthTrueIndex}(l, r, x) \to \tuple''_x = c_{l,r} \land \\

\bigland\limits_{x=1}^{\sum\limits_{i=1}^{u} \indicator(b_i)} \land_{i=1}^u b_i \to \land_{k=1}^{p} \denot{a_{k}}_{\schema, \symdb, [\tuple''_{N + x}]} = \denot{a_{k}}_{\schema, \symdb, [\tuple_{i}]} \land \land_{k=1}^{q} \denot{a_{k}'}_{\schema, \symdb, [\tuple''_{N + x}]} = \nullv

\end{array}}
{\schema, \symdb \vdash \ljoin(\relation_1, \relation_2, \phi) \Downarrow \relation' \leadsto \formula}
{\text{(LeftJoin)}}

\end{array}
\]
\caption{Underapproximate semantics. findNthTrueIndex(l, r, n) finds the $p_{l,r}$ that is the $n$th $p_{i,j}$ evaluates to $\top$, defined formally as $\exists l, r. p_{l,r} = \top \land \sum_{i=1}^l \sum_{j=1}^r \indicator(p_{l, r} = \top) = n$}
\label{fig:stale-under-semantics}
\end{figure}

